A C-13(alpha,n)O-16 calibration source for KamLAND

We report on the construction and performance of a calibration source for KamLAND using the reaction C-13(alpha,n)O-16 with Po-210 as the alpha progenitor. The source provides a direct measurement of this background reaction in our detector, high energy calibration points for the detector energy scale, and data on quenching of the neutron visible energy in KamLAND scintillator. We also discuss the possibility of using the reaction C-13(alpha,n)O-16 as a source of tagged slow neutrons.

==> Makefile <==
# 14 June 2003  David McKee
#
# This is to simpilfy the building: repeated running to 
# get the refrences right, cleanup of miscelaneous files, etc...
SH=/bin/bash
LATEX=latex
BIBTEX=bibtex
MAKEINDEX=makeindex
DVIPS=dvips -t LetterSize 
DVIPDF=dvipdfm -p letter
PDF2PS = pdf2ps
PS2PDF = pstopdf 
#ps2pdf
PDFTEX=pdflatex
TAR=tar
RM=rm -f

# Needed for the tarba
HERE=nim_c13source


ROOTNAME=nim_c13source
MAIN=$(ROOTNAME).tex
DVI=$(ROOTNAME).dvi
PS=$(ROOTNAME).ps
PDF=$(ROOTNAME).pdf
TARBAL=$(ROOTNAME).tgz
XXXTARBAL=../$dmckee_$(ROOTNAME)_arXive.tar.gz

basic: $(DVI) 

all: refs ps


# Build a device independant file
dvi: $(DVI)

$(DVI): $(MAIN)
	$(LATEX) $(MAIN)



# make refs should either:
#
#    ==> *.dvi more recent than *.tex: latex again to insure the 
#        references are right
#    ==> *.tex more recent than *.dvi: latex twice
refs: $(DVI)
	$(LATEX) $(MAIN)

ps: $(PS)

$(PS): $(DVI)
	$(DVIPS) -o $@ $^

pdf: $(PDF)

$(PDF): $(DVI)
	$(DVIPDF) -o $@ $^
#	$(PS2PDF) $(PS) 
#	$(PDFTEX) $(MAIN)


# diagrams: cleandiagrams
# 	mf '\mode:=ljfour; input g0_talk_diagrams_mf'

# cleandiagrams :
# 	rm -f g0_talk_diagrams_mf.tfm
# 	rm -f g0_talk_diagrams_mf.[0-9]*gf
# 	rm -f g0_talk_diagrams_mf.[0-9]*pk
# 	rm -f g0_talk_diagrams_mf.t[1234567]
# 	rm -f g0_talk_diagrams_mf.log


# TARBALL makers.
#
# tarbal includes the dvi, ps and pdf files, sourcetar gives only the 
# source files (includeing this makefile)
tarbal : clean tarbase

sourcetar : scrub tarbase

tarbase : 
	make -e dotar

dotar :
	(cd ..; $(TAR) czf $(TARBAL) $(HERE))

xxxtarbal: 
	$(TAR) czf $(XXXTARBAL) $(MAIN) fig*.eps

# Cleanup.
clean :
	$(RM) *.aux *.ind *.idx *.log *.toc *.lof *.lot *.ilg *~ core

cleaner: clean
	$(RM) $(DVI) *.bbl *.blg

scrub: cleaner #cleandiagrams 
#	$(RM) g0_talk_diagrams_mf.mf
	$(RM) $(PS) $(PDF)


